Continuous Release of Data Streams under both Centralized and Local Differential Privacy

In this paper, we study the problem of publishing a stream of real-valued data satisfying differential privacy (DP). One major challenge is that the maximal possible value can be quite large; thus it is necessary to estimate a threshold so that numbers above it are truncated to reduce the amount of noise that is required to all the data. The estimation must be done based on the data in a private fashion. We develop such a method that uses the Exponential Mechanism with a quality function that approximates well the utility goal while maintaining a low sensitivity. Given the threshold, we then propose a novel online hierarchical method and several post-processing techniques. Building on these ideas, we formalize the steps into a framework for private publishing of stream data. Our framework consists of three components: a threshold optimizer that privately estimates the threshold, a perturber that adds calibrated noises to the stream, and a smoother that improves the result using post-processing. Within our framework, we design an algorithm satisfying the more stringent setting of DP called local DP (LDP). To our knowledge, this is the first LDP algorithm for publishing streaming data. Using four real-world datasets, we demonstrate that our mechanism outperforms the state-of-the-art by a factor of 6-10 orders of magnitude in terms of utility (measured by the mean squared error of answering a random range query).

==> app_algorithms.tex <==

\section{Detailed Algorithm Description}
\label{app:alg}
We summarize the algorithms of \method with necessary details in \autoref{alg:ToPS2}.  We first cache the first $m$ values and obtain $\theta$.  Then for each of the following value, we first truncate it and then use the hierarchical method together with the smoother to output the noisy value.  


\begin{algorithm}[h]
\footnotesize
\LinesNumbered
\caption{\method}
\label{alg:ToPS2}

\KwIn{$V=\langle v_1, v_2, \ldots\rangle$, $\epsilon$, $m$, upper bound on query range $r$}
\KwOut{$\tilde{V}=\langle \tilde{v}_1, \tilde{v}_2, \ldots\rangle$}


$V_m \gets \langle v_1, \ldots v_m\rangle$ \tcp*{Cache $m$ values}

\For{$\theta = 1$ to $B$}{
 $m_\theta\gets |\{i\mid v_i \le \theta, i\in[m] \}|$ \tcp*{\autoref{eq:m}}
 
 $q_\theta(V_m) \gets -\frac{m \theta}{20 r\epsilon}\sqrt{2(b-1)\log_b^3(r)} - m_\theta$ \tcp*{\autoref{eq:eme_q}}
 
 $\tilde{q}_\theta(V) = q_\theta(V_m) + \Lapp{\frac{1}{\epsilon}}$ \tcp*{$\mathsf{GS}_g=1$, $q$ is monotonic}
 }
 
 
 $\theta \gets \argmax_\theta \tilde{q}_\theta(V) $ 
   \tcp*{Find $\theta$ via Noisy Max (\autoref{subsec:dp_primitive})}
 
  \tcc{The previous part of the code finds $\theta$. \\
  Now we are ready to release the stream.}
 
   
 $h\gets \log_{16} r$ $;$
 
 $s \gets \argmin_s \left[15\left(\log_{16}(r)-s\right)^3\frac{2\theta^2}{\epsilon^2} + \frac{16^{2s}}{4}\frac{\theta^2}{9}\right]$ \tcp*{\autoref{eq:mse_guess}}
 
 $u\gets \frac{16^s\theta}{2}$ $;$
 
 $build \gets $ True \tcp*{Indicator to build a tree}
 
 \ForEach{$i>m$}{
   $v_i \gets \min(v_i, \theta)$ \tcp*{Truncate}
   
   \uIf {\text{build}}{
     Init an $(h-s)$-layer hierarchy with fan-out $16$ $;$
     
     Assign $0$ to all nodes \tcp*{Build the virtual tree}
     
     Add $\Lapp{\frac{h-s}{\epsilon}}$ to each node $;$
     
     Make the tree consistent \tcp*{\autoref{app:consist}}
     
     $cur\_node \gets$ left-most noisy node on tree $;$
     
     $build \gets $ False $;$
   }
   
   \uIf {$(i - m) \% r = 0$}{
     $build \gets $ True \tcp*{Time to build another tree}
   }
   
   \uIf {$(i - m) \% 16^s = 0$}{
     
     {\bf Output} $cur\_node - u \times (16^s - 1)$ $;$
     
     $u_t \gets cur\_node $ $;$
     
     $cur\_node\gets$ next noisy node on tree $;$
   }
   \uElse{
     
     {\bf Output} $u/16^s$ \tcp*{``Recent'' smoother in \autoref{app:smooth}}
     
     $cur\_node\gets cur\_node+ v_i$ $;$
   }
} 
\end{algorithm}


% \begin{algorithm}[th]
% \footnotesize
% \LinesNumbered
% \caption{\methodldp}
% \label{alg:ToPL}

% \KwIn{Raw value $v$, private budget $\epsilon$}
% \KwOut{Private value $\tilde{v}$}

% Estimate threshold $\theta$ in the range of $[0,B]$ by optimizing error formula \autoref{eq:range_error_ldp} using \SW as a white box (SW-W) in \autoref{sec:method_ldp};

% \uIf{$v > \theta$}{
%     Set $v \gets \theta$ \;
%   }
% Release private value $\tilde{v}$ using Hybrid Mechanism (see \autoref{app:ldp_fo}) with $\epsilon$.


% \end{algorithm}



% \begin{algorithm}[th]
% \footnotesize
% \LinesNumbered
% \caption{\method}
% \label{alg:ToPS}

% \KwIn{Raw stream $V=\langle v_1, v_2, \ldots\rangle$, privacy budget $\epsilon$, time lag $m$, fan-out $b$, upper bound on query range $r$;}
% \KwOut{Private stream $\tilde{V}=\langle \tilde{v}_1, \tilde{v}_2, \ldots\rangle$;}

% Estimate threshold $\theta$ in the range of $[0,B]$
% based on the first $m$ values using Exponential mechanism with quality function $q(V,\theta) = -\frac{3m \theta}{c r\epsilon}\sqrt{2(b-1)\log_b^3(r)} - m_\theta$ (see \autoref{eq:eme_q});

%  \For{$i>m$}{
%     \uIf{$v_i$ > $\theta$}{
%     Set $v_i \gets \theta$ \;
%   }
%  Construct an $h$-layer hierarchy with fan-out $b$ from $\langle v_{m+1}, v_{m+2}, \ldots\rangle$ (from each $r$ values, if infinite stream);
 
%  For each leaf/node $x$, add noise from Laplace mechanism using the online consistency algorithm in \autoref{app:consist} with an $\epsilon/h$ to each layer, which yields $\epsilon$-DP;
 
%  Optimize smoother parameter $s$ by minimizing error formula:
%  $(b-1)\left(\log_b(r)-s\right)^3\frac{2\theta^2}{\epsilon^2} + \frac{b^s}{2}\frac{\theta^2}{4}$ (see \autoref{eq:mse_guess});

% Replace output of $s$ lower levels of the hierarchy using smoother ``Recent'' (see \autoref{app:smooth}).
%     } 
% \end{algorithm}

==> app_gauss.tex <==
\section{No Benefit of Introducing $\delta$}
\label{subsec:delta}
We propose to use the Laplace mechanism in this paper.  For completeness, we also describe the Gaussian mechanism, which is more frequently used in differentially private machine learning~\cite{ccs:abadi2016deep,iclr:papernot2018scalable}.  The advantage of using the Gaussian mechanism is that its sensitivity $\mathsf{GS}$ is defined on $L_2$ norm, and it can better enjoy the modern composition theorems.  Below we first give a detailed description of the Gaussian mechanism and the composition theorems.  

\begin{table*}[!h]
\centering
\caption{Comparison of variance of noise under different number of compositions, fixing $\mathsf{GS}=1$ and $\delta=10^{-9}$}
\label{tbl:noise_eps}
\begin{tabular}{@{}c|c|c|c|c|c|c|c|c@{}}
\toprule
$\epsilon$ & Mechanism, composition & $k=5$ & $k=10$ & $k=15$ & $k=20$ & $k=30$ & $k=50$ & $k=100$\\ \midrule
\multirow{4}{*}{$0.01$} &Laplace, sequential & 	5.0E+05& 	2.0E+06& 	4.5E+06& 	8.0E+06	& 1.8E+07	& 5.0E+07& 	2.0E+08	\\
&Laplace, advanced & 
 4.1E+06& 	8.3E+06	& 1.2E+07& 	1.7E+07& 	2.5E+07	& 4.1E+07& 	8.3E+07	\\
&Gauss, advanced & 
 	1.0E+08	& 2.1E+08& 	3.1E+08& 	4.2E+08	& 6.4E+08	& 1.1E+09	& 2.2E+09	\\
&Gauss, \zcdp & 
 	2.1E+06& 	4.1E+06	& 6.2E+06& 	8.3E+06	& 1.2E+07& 	2.1E+07& 	4.1E+07	\\\midrule
\multirow{4}{*}{$0.1$} &Laplace, sequential & 
5.0E+03&	2.0E+04	&4.5E+04&	8.0E+04&	1.8E+05	&5.0E+05&	2.0E+06	\\
&Laplace, advanced & 
4.2E+04&	8.3E+04	&1.2E+05&	1.7E+05	&2.5E+05&	4.2E+05&	8.3E+05	\\
&Gauss, advanced & 
1.0E+06	&2.1E+06&	3.1E+06&	4.2E+06&	6.5E+06&	1.1E+07&	2.3E+07	\\
&Gauss, \zcdp & 
	2.1E+04&	4.2E+04	&6.2E+04&	8.3E+04&	1.2E+05&	2.1E+05	&4.2E+05	\\\midrule
\multirow{4}{*}{$1$} &Laplace, sequential & 
5.0E+01&	2.0E+02&	4.5E+02&	8.0E+02	&1.8E+03&	5.0E+03	&2.0E+04	\\
&Laplace, advanced & 
4.3E+02&	8.7E+02&	1.3E+03&	1.7E+03	&2.6E+03&	4.3E+03&	8.7E+03	\\
&Gauss, advanced & 
1.0E+04&	2.1E+04	&3.3E+04&	4.4E+04	&6.7E+04&	1.1E+05&	2.4E+05	\\
&Gauss, \zcdp & 
2.1E+02&	4.2E+02	&6.4E+02&	8.5E+02	&1.3E+03&	2.1E+03	&4.2E+03	\\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[!h]
\centering
\caption{Comparison of variance of noise under different number of compositions, fixing $\epsilon=0.01$ and $\delta=10^{-9}$.}
\label{tbl:noise_sensitivity}
\begin{tabular}{@{}c|c|c|c|c|c|c|c|c@{}}
\toprule
$\mathsf{GS}$ & Mechanism, composition & $k=5$ & $k=10$ & $k=15$ & $k=20$ & $k=30$ & $k=50$ & $k=100$\\ \midrule
\multirow{4}{*}{$10$} &Laplace, sequential & 	5.0E+07	& 2.0E+08	& 4.5E+08	& 8.0E+08	& 1.8E+09	& 5.0E+09	& 2.0E+10	\\
&Laplace, advanced &   4.1E+08	& 8.3E+08	& 1.2E+09	& 1.7E+09	& 2.5E+09	& 4.1E+09	& 8.3E+09	\\
&Gauss, advanced &  1.0E+10	& 2.1E+10	& 3.1E+10	& 4.2E+10	& 6.4E+10	& 1.1E+11	& 2.2E+11	\\
&Gauss, \zcdp &   2.1E+08	& 4.1E+08	& 6.2E+08	& 8.3E+08	& 1.2E+09	& 2.1E+09	& 4.1E+09	\\\midrule
\multirow{4}{*}{$100$} &Laplace, sequential &  5.0E+09	& 2.0E+10	& 4.5E+10	& 8.0E+10	& 1.8E+11	& 5.0E+11	& 2.0E+12	\\
&Laplace, advanced & 4.1E+10	& 8.3E+10	& 1.2E+11	& 1.7E+11	& 2.5E+11	& 4.1E+11	& 8.3E+11	\\
&Gauss, advanced &  1.0E+12	& 2.1E+12	& 3.1E+12	& 4.2E+12	& 6.4E+12	& 1.1E+13	& 2.2E+13	\\
&Gauss, \zcdp &2.1E+10	& 4.1E+10	& 6.2E+10	& 8.3E+10	& 1.2E+11	& 2.1E+11	& 4.1E+11	\\
\bottomrule
\end{tabular}
\end{table*}


\begin{table*}[!h]
\centering
\caption{Comparison of variance of noise under different number of compositions, fixing $\epsilon=0.01$ and $\mathsf{GS}=1$.}
\label{tbl:noise_delta}
\begin{tabular}{@{}c|c|c|c|c|c|c|c|c@{}}
\toprule
$\delta$ & Mechanism, composition & $k=5$ & $k=10$ & $k=15$ & $k=20$ & $k=30$ & $k=50$ & $k=100$\\ \midrule
\multirow{4}{*}{$10^{-12}$} &Laplace, sequential &  5.0E+05	& 2.0E+06	& 4.5E+06	& 8.0E+06	& 1.8E+07	& 5.0E+07	& 2.0E+08	\\
&Laplace, advanced &  5.5E+06	& 1.1E+07	& 1.7E+07	& 2.2E+07	& 3.3E+07	& 5.5E+07	& 1.1E+08	\\
&Gauss, advanced &   1.7E+08	& 3.5E+08	& 5.3E+08	& 7.1E+08	& 1.1E+09	& 1.8E+09	& 3.8E+09	\\
&Gauss, \zcdp & 2.8E+06	& 5.5E+06	& 8.3E+06	& 1.1E+07	& 1.7E+07	& 2.8E+07	& 5.5E+07	\\\midrule
\multirow{4}{*}{$10^{-15}$} &Laplace, sequential &   5.0E+05	& 2.0E+06	& 4.5E+06	& 8.0E+06	& 1.8E+07	& 5.0E+07	& 2.0E+08	\\
&Laplace, advanced &  6.9E+06	& 1.4E+07	& 2.1E+07	& 2.8E+07	& 4.1E+07	& 6.9E+07	& 1.4E+08	\\
&Gauss, advanced &  2.6E+08	& 5.3E+08	& 8.1E+08	& 1.1E+09	& 1.6E+09	& 2.8E+09	& 5.6E+09	\\
&Gauss, \zcdp &  3.5E+06	& 6.9E+06	& 1.0E+07	& 1.4E+07	& 2.1E+07	& 3.5E+07	& 6.9E+07	\\
\bottomrule
\end{tabular}
\end{table*}


\input{primitive_gau}

\input{primitive_zcdp}


\mypara{Comparison of Composition Techniques}
In \autoref{tbl:noise_eps}, we show the expected noise scale (variance) of an individual subroutine under different settings, varying the number of compositions $k$ from $1$ to $100$, and fixing sensitivity $\mathsf{GS}_f=1$ and $\delta=10^{-9}$.
From the table, we can see that regardless of the setting, noise always grows as $k$ increases, or as $\epsilon$  decreases.
%From the Table, we can see that from left to right, noise grows with $k$; and from top to bottom, noise decreases with $\epsilon$.  Note that regardless of $k$, the scale of noise is always 
Comparing the rows, it is interesting to see that the noise scale (variance) is proportional to $1/\epsilon^2$.  

A similar effect also appears in \autoref{tbl:noise_sensitivity}, when we change the sensitivity $\mathsf{GS}$ to $10$ and $100$, while fixing $\epsilon=0.01$.  Together with \autoref{tbl:noise_eps}, we can see that regardless of composition, the scale of noise is proportional to $\mathsf{GS}^2/\epsilon^2$.

\autoref{tbl:noise_delta} shows the noise scale varying $\delta$.  Comparing the numbers here with those in the first group of rows in \autoref{tbl:noise_eps}, we can see that reducing $\delta$ does not affect the Laplace mechanism with sequential composition, but incurs larger noise to other settings.  It is less clear though what is the relation between $\delta$ and noise, because $\delta$ appears in the logarithm function.


For the specific mechanism and composition technique, we can see Laplace mechanism with sequential composition works best up to $k=20$, and this holds in all $\epsilon$ and $\mathsf{GS}$ settings in \autoref{tbl:noise_eps} and~\autoref{tbl:noise_sensitivity}.  If we reduce $\delta$, as shown in \autoref{tbl:noise_delta}, the turning point of $k$ for which the Laplace mechanism with sequential composition becomes sub-optimal becomes larger.
As in our paper, the composition is typically small, we choose to use the Laplace mechanism with sequential composition.  When $k$ becomes larger, we can see that the Gaussian mechanism with \zcdp composition introduces the least amount of noise.  For the other two approaches with advanced composition, they are always worse than \zcdp composition; and the Laplace mechanism works better than the Gaussian mechanism up to $k=100$.



==> app_update_thres.tex <==
\section{Different Ways of Updating $\tau$}
\label{app:update_thres}
We decompose the problem of updating $\tau$ into three sub-problems: (1) decide when to update; (2) which direction should we change $\tau$; and (3) how much is the change.  We first analyze the general problem of {\it deciding above or below}.




\mypara{Above or Below}
We want to decide whether the desired threshold is above or below the old threshold.  There are two methods to do it: (1) using Laplace mechanism to publish the value, and then compare the noisy value with the threshold; and (2) using EM to output either above or below.  Intuitively, the second technique may be better because it gives the minimal information (only one bit).  To formally compare the two methods, we calculate the probability the correct answer is generated.  Suppose the private value is $t$, and the threshold is $T$, we have:
In LM, the output is $t+\eta$ where $\eta = \Lapp{\frac{1}{\epsilon}}$ (sensitivity is $1$).  Given $t>T$ (denote $b=t-T$), 
\begin{align}
    \Pr{t+\eta > T} = \Pr{\eta > T - t} = 1 - \Pr{\eta < T - t} =  \frac{1}{2}\exp{\left(-(T-t)\epsilon\right)} =  \frac{1}{2}\exp{\left(b\epsilon\right)}\label{eq:lm_correct_prob}
\end{align}

% As $\Pr{\Lapp{\frac{1}{\epsilon}}=x}  = \frac{1}{2\beta} \myexp{-|x|\epsilon}$
    
    
For EM, we define the quality function for outputting $+1$ or $-1$ as
\begin{align*}
    q_{+1}(D) = t - T \\
    q_{-1}(D) = T - t
\end{align*} 

This gives the probability of outputting $+1$ to be
\begin{align}
     \Pr{\AA_q(t)=+1} = \frac{\exp{\left(\frac{\epsilon b }{2}\right)}}{\exp{\left(\frac{\epsilon b}{2}\right)} + \exp{\left(\frac{-\epsilon b}{2}\right)}} = \frac{\exp{\left(\epsilon b\right)}}{\exp{\left(\epsilon b\right)} + 1}\label{eq:em_correct_prob}
\end{align}
Comparing Equation~\eqref{eq:lm_correct_prob} with Equation~\eqref{eq:em_correct_prob}, we have \eqref{eq:lm_correct_prob} is always greater than \eqref{eq:em_correct_prob} because $\exp{\left(b\epsilon\right)} > 1$.  Note that even if the quality functions in EM are monotonic, this still holds.  Thus Laplace mechanism always performs better.
Moreover, we can extend the method with a ``buffer''.  That is, if $t$ is close to $T$, we allow the output of $0$.


\begin{algorithm}[!htb]
	\caption{Find how to update $\ell$}\label{algo:svt_tau_bi}
	\begin{algorithmic}[1]
		\Function{UpdateLimit}{$V, \epsilon, \tau$} 
    		\State $\epsilon_1 \gets \frac{\epsilon}{2}, \epsilon_2 \gets \frac{\epsilon}{2}, \mathsf{GS}_q \gets 1$
    		\State $\rho \gets \Lapp{\frac{\mathsf{GS}_q}{\epsilon_1}}$
    		\For {$i = 1$ to $+\infty$}
		        \State $q_{i,1}(V) \gets p \cdot |V| - |\{j\mid v_j \le \ell_m - (i - 1) \}|$
		        \If {$q_{i,1}(V) + \Lapp{\frac{2\mathsf{GS}_q}{\epsilon_2}} \ge \rho$}
                    \State \Return $i,1$
                \EndIf
		        \State $q_{i,2}(V) \gets |\{j\mid v_j \le i \}| - p \cdot |V|$
                \If {$q_{i,2}(V) + \Lapp{\frac{2\mathsf{GS}_q}{\epsilon_2}} \ge \rho$}
                    \State \Return $i,2$
                \EndIf
    		\EndFor
	    \EndFunction
	\end{algorithmic}
\end{algorithm}


\mypara{How Much to Change}
Having decided whether to go up or down, we can then decide how much change we want to apply to $\tau$.  Setting a pre-defined change quantity helps when the change is predictable, but when the data change drastically, using SVT to obtain it seems more reasonable.  Note that it is also possible to decide the new $\tau$ (both direction and step) at once.  We thus have the following options:
\begin{itemize}
    \item Algorithm~\ref{algo:svt_tau}.  Note that this does not utilize the information of the last $\tau$.
    \item Using SVT but searching for two directions, starting from $1$ and $\ell_m$.  In particular, we define the sequence of queries
    \begin{align*}
        q_{i,1}(V) &=  p \cdot |V| - |\{j\mid v_j \le \ell_m - (i - 1)\}| , \\
        q_{i,2}(V) &= |\{j\mid v_j \le i\}| - p \cdot |V| .
    \end{align*}
    Algorithm~\ref{algo:svt_tau_bi} gives the full procedure.  Note that the queries are no longer monotonic.   
    % Although this utilizes the last $\tau$, this may not help, as the current $\tau$ may be far from the previous $\tau$.  In some cases, this gives worse result than the naive Algorithm~\ref{algo:svt_tau} (e.g., when the current $\tau$ is small and the previous $\tau$ is large).  
    \item First decide whether the desired $\tau$ is above or below the currently used $\tau$, and then use SVT but searching with only one direction from $\tau$.  That is,
    \begin{align*}
        q_i(V) &=  p \cdot |V| - |\{j\mid v_j \le \tau - i\}| &\mbox{ if we want to decrease}, \\
        q_i(V) &= |\{j\mid v_j \le \tau + i\}| - p \cdot |V| &\mbox{ if we want to increase}.
    \end{align*}
\end{itemize}

Compared to the third option, the second option searches in one wrong direction, note that the third option also spend some privacy budget in determining the direction.  Which method is better actually depends on the underlying data.  Intuitively, if the desired $\tau$ is larger than the previous $\tau$, method (3) trades-off some privacy budget to save the initial searches.  If on the other hand, it is smaller and closer to the starting point, method (1) will be better.


\mypara{When to Update}
% Given the technique to test whether the threshold is set too high or too low, we then investigate when should this test be used, how frequent it should be used.
We can always update  $\tau$ periodically.  On the other hand, we can also decide whether or not to update based on the observed noisy counts.  For example, one heuristic could be to test whether the mean of the noisy counts is close to the threshold.  What is more interesting is to use SVT for this test.  In particular, at each observation, we test whether we should change $\tau$.  Here we use a threshold $\theta$; and if the desired $\tau$ deviates from the previous one by more than $\theta$, we want to update it.  There are several variants we can consider:


\begin{itemize}
    \item Testing whether the $\tau$ so far deviates from the previous one by a large amount.  In particular, define the sequence of queries
    \begin{align*}
        q_i(V) &= \max(|\{j\mid v_j\le \tau, j \le i\}| - p i, 0) - \theta i
    \end{align*}
    Note that each query takes a prefix of the observations $v_1$ till $v_i$, while previous discussions focus on fixing the observations.  The procedure is presented in Algorithm~\ref{algo:svt_tau_update}.  
    
    \item Detect both when to update $\tau$ and the direction (above or below) together.  That is, define the sequence of queries
    \begin{align*}
        q_{i,1}(V) &= |\{j\mid v_j \le \tau, j \le i\}| - (p+\theta) i, \\
        q_{i,2}(V) &= (p-\theta) i - |\{j\mid v_j \le \tau, j \le i\}|.
    \end{align*}
    The procedure is presented in Algorithm~\ref{algo:svt_tau_update_bi}.  
    
    \item Finally, we can detect when, which direction, and how much to change $\tau$ in one SVT.  The idea is to extend each query of Algorithm~\ref{algo:svt_tau_update_bi} with a sequence of queries (from the idea of Algorithm~\ref{algo:svt_tau_bi}).  In particular,
    \begin{align*}
        q_{i,1,j}(V) &= |\{k\mid v_k \le \min(j,\tau), k \le i\}| - (p+\theta) i, \\
        q_{i,2,j}(V) &= (p-\theta) i - |\{k\mid v_k \le \max(\ell_m+1-j,\tau), k \le i\}|.
    \end{align*}
\end{itemize}
After the algorithm returns, one can resume it with the rest of the observations.

Overall, it is desired to start warm, because we have to use the threshold up front, and without sufficient observations, it cannot be reliably determined.  That is, we may update more frequently from the beginning, and less frequently later.

How many observations we use for this test is another aspect to consider.  Intuitively, the more data, the better the result will be.  However, some data may be obsolete and thus influence with the result. 



\begin{algorithm}[!htb]
	\caption{Find when to update $\tau$}\label{algo:svt_tau_update}
	\begin{algorithmic}[1]
		\Function{UpdateLimit}{$V, \epsilon, \tau$} 
    		\State $\epsilon_1 \gets \frac{\epsilon}{2}, \epsilon_2 \gets \frac{\epsilon}{2}, \mathsf{GS}_q \gets 1$
    		\State $\rho \gets \Lapp{\frac{\mathsf{GS}_q}{\epsilon_1}}$
    		\For {$i = 1$ to $+\infty$}
		        \State $q_i(V) \gets \max(|\{j\mid v_j\le \tau, j \le i\}| - p i, 0) - \theta i$
                \If {$q_i(V) + \Lapp{\frac{2\mathsf{GS}_q}{\epsilon_2}} \ge \rho$}
                    \State \Return $i$
                \EndIf
    		\EndFor
	    \EndFunction
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}[!htb]
	\caption{Find when and how to update $\ell$}\label{algo:svt_tau_update_bi}
	\begin{algorithmic}[1]
		\Function{UpdateLimit}{$V, \epsilon, \tau$} 
    		\State $\epsilon_1 \gets \frac{\epsilon}{2}, \epsilon_2 \gets \frac{\epsilon}{2}, \mathsf{GS}_q \gets 1$
    		\State $\rho \gets \Lapp{\frac{\mathsf{GS}_q}{\epsilon_1}}$
    		\For {$i = 1$ to $+\infty$}
		        \State $q_{i,1}(V) \gets|\{j\mid v_j \le \tau, j \le i\}| - (p+\theta) i$
                \If {$q_{i,1}(V) + \Lapp{\frac{2\mathsf{GS}_q}{\epsilon_2}} \ge \rho$}
                    \State \Return $i,1$
                \EndIf
		        \State $q_{i,2}(V) \gets (p-\theta) i - |\{j\mid v_j \le \tau, j \le i\}|$
                \If {$q_{i,2}(V) + \Lapp{\frac{2\mathsf{GS}_q}{\epsilon_2}} \ge \rho$}
                    \State \Return $i,2$
                \EndIf
    		\EndFor
	    \EndFunction
	\end{algorithmic}
\end{algorithm}

==> figure/old/b-tree.tex <==


\begin{figure}[ht]

\usepackage{tikz}
\usetikzlibrary{arrows, calc, patterns}

\tikzset{
  treenode/.style = {align=center, inner sep=0pt, text centered,
    font=\sffamily},
  arn_n/.style = {treenode, circle, white, font=\sffamily\bfseries, draw=black,
    fill=black, text width=1.5em},% arbre rouge noir, noeud noir
  arn_r/.style = {treenode, circle, red, draw=red, 
    text width=1.5em, very thick},% arbre rouge noir, noeud rouge
  arn_x/.style = {treenode, rectangle, draw=black,
    minimum width=0.5em, minimum height=0.5em}% arbre rouge noir, nil
}

\begin{center}
\begin{tikzpicture}[->,>=stealth',level/.style={sibling distance = 4.1cm/#1,
 level distance = 0.7cm}] 
\node [arn_r] {}
    child{ node [arn_n] {} 
            child{ node [arn_r] {} 
            	child{ node [arn_r] {1} }
            	child{ node [arn_r] {2}}
            }
            child{ node [arn_r] {} 
            	child{ node [arn_r] {3} }
            	child{ node [arn_r] {4}}
            }                            
    }
    child{ node [arn_r] {} 
            child{ node [arn_n] {} 
            	child{ node [arn_r] {5} }
            	child{ node [arn_r] {6}}
            }
            child{ node [arn_r] {} 
            	child{ node [arn_n] {7} }
            	child{ node [arn_r] {8}}
            }                            
    }
; 
\end{tikzpicture}
\end{center}

\caption{Example of the binary tree algorithm~\cite{cont-observe, cont-release}. To compute the sum of the first 7 observations, noise is added to only 3 nodes whose union equals the interval $[1, 7]$.}
\label{fig:binary-tree}
\end{figure}

==> figure/old/eps1_ratio.tex <==



\begin{figure*}[ht]
	\centering
	\subfigure[time, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/time_eps1m50000p850_ell}
	}
	\subfigure[fare, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/fare_eps1m50000p850_ell}
	}
	\subfigure[dist, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/dist_eps1m50000p850_ell}
	}
	
	\centering
	\subfigure[time, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/time_eps1m50000p950_ell}
	}
	\subfigure[fare, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/fare_eps1m50000p950_ell}
	}
	\subfigure[dist, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/dist_eps1m50000p950_ell}
	}
	
	\centering
	\subfigure[time, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/time_eps1m50000p995_ell}
	}
	\subfigure[fare, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/fare_eps1m50000p995_ell}
	}
	\subfigure[dist, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/dist_eps1m50000p995_ell}
	}
	\caption{Empirical average error of percentile estimation.   $\epsilon=0.1$.}
\end{figure*}


\begin{figure*}[ht]
	\centering
	\subfigure[time, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/time_eps1m50000p850_ell_perc_dist}
	}
	\subfigure[fare, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/fare_eps1m50000p850_ell_perc_dist}
	}
	\subfigure[dist, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/dist_eps1m50000p850_ell_perc_dist}
	}
	
	\centering
	\subfigure[time, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/time_eps1m50000p950_ell_perc_dist}
	}
	\subfigure[fare, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/fare_eps1m50000p950_ell_perc_dist}
	}
	\subfigure[dist, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/dist_eps1m50000p950_ell_perc_dist}
	}
	
	\centering
	\subfigure[time, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/time_eps1m50000p995_ell_perc_dist}
	}
	\subfigure[fare, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/fare_eps1m50000p995_ell_perc_dist}
	}
	\subfigure[dist, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/dist_eps1m50000p995_ell_perc_dist}
	}
	\caption{Empirical average error of percentile estimation.   $\epsilon=0.1$.}
\end{figure*}


\begin{figure*}[ht]
	\centering
	\subfigure[kosarak, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/kosarak_eps1m50000p850_ell}
	}
	\subfigure[pos, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/pos_eps1m50000p850_ell}
	}
	\subfigure[retail, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/retail_eps1m50000p850_ell}
	}
	
	\centering
	\subfigure[kosarak, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/kosarak_eps1m50000p950_ell}
	}
	\subfigure[pos, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/pos_eps1m50000p950_ell}
	}
	\subfigure[retail, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/retail_eps1m50000p950_ell}
	}
	
	\centering
	\subfigure[kosarak, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/kosarak_eps1m50000p995_ell}
	}
	\subfigure[pos, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/pos_eps1m50000p995_ell}
	}
	\subfigure[retail, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/retail_eps1m50000p995_ell}
	}
	\caption{Empirical average error of percentile estimation.   $\epsilon=0.1$.}
\end{figure*}


\begin{figure*}[ht]
	\centering
	\subfigure[kosarak, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/kosarak_eps1m50000p850_ell_perc_dist}
	}
	\subfigure[pos, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/pos_eps1m50000p850_ell_perc_dist}
	}
	\subfigure[retail, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/retail_eps1m50000p850_ell_perc_dist}
	}
	
	\centering
	\subfigure[kosarak, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/kosarak_eps1m50000p950_ell_perc_dist}
	}
	\subfigure[pos, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/pos_eps1m50000p950_ell_perc_dist}
	}
	\subfigure[retail, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/retail_eps1m50000p950_ell_perc_dist}
	}
	
	\centering
	\subfigure[kosarak, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/kosarak_eps1m50000p995_ell_perc_dist}
	}
	\subfigure[pos, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/pos_eps1m50000p995_ell_perc_dist}
	}
	\subfigure[retail, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/retail_eps1m50000p995_ell_perc_dist}
	}
	\caption{Empirical average error of percentile estimation.   $\epsilon=0.1$.}
\end{figure*}




\begin{figure*}[ht]
	\centering
	\subfigure[web1, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/web1_eps1m50000p850_ell}
	}
	\subfigure[web2, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/web2_eps1m50000p850_ell}
	}
	\subfigure[star, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/star_eps1m50000p850_ell}
	}
	
	\centering
	\subfigure[web1, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/web1_eps1m50000p950_ell}
	}
	\subfigure[web2, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/web2_eps1m50000p950_ell}
	}
	\subfigure[star, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/star_eps1m50000p950_ell}
	}
	
	\centering
	\subfigure[web1, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/web1_eps1m50000p995_ell}
	}
	\subfigure[web2, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/web2_eps1m50000p995_ell}
	}
	\subfigure[star, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/star_eps1m50000p995_ell}
	}
	\caption{Empirical average error of percentile estimation.   $\epsilon=0.1$.}
\end{figure*}



\begin{figure*}[ht]
	\centering
	\subfigure[web1, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/web1_eps1m50000p850_ell_perc_dist}
	}
	\subfigure[web2, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/web2_eps1m50000p850_ell_perc_dist}
	}
	\subfigure[star, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/star_eps1m50000p850_ell_perc_dist}
	}
	
	\centering
	\subfigure[web1, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/web1_eps1m50000p950_ell_perc_dist}
	}
	\subfigure[web2, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/web2_eps1m50000p950_ell_perc_dist}
	}
	\subfigure[star, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/star_eps1m50000p950_ell_perc_dist}
	}
	
	\centering
	\subfigure[web1, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/web1_eps1m50000p995_ell_perc_dist}
	}
	\subfigure[web2, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/web2_eps1m50000p995_ell_perc_dist}
	}
	\subfigure[star, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/eps1_ratio/star_eps1m50000p995_ell_perc_dist}
	}
	\caption{Empirical average error of percentile estimation.   $\epsilon=0.1$.}
\end{figure*}

==> figure/old/nyc_ell.tex <==
\begin{figure*}[ht]
	\centering
	\subfigure[Time, 0.85, 1411, 1295]{
		\includegraphics[width=0.31\textwidth]{figure/s/time_eps1m50000p850_ell}
	}
	\subfigure[Fare, 0.85, 525, 440]{
		\includegraphics[width=0.31\textwidth]{figure/s/fare_eps1m50000p850_ell}
	}
	\subfigure[Distance, 0.85, 525, 440]{
		\includegraphics[width=0.31\textwidth]{figure/s/dist_eps1m50000p850_ell}
	}
	
	\centering
	\subfigure[Time, 0.95, 1928, 1959]{
		\includegraphics[width=0.31\textwidth]{figure/s/time_eps1m50000p950_ell}
	}
	\subfigure[Fare, 0.95, 860, 1036]{
		\includegraphics[width=0.31\textwidth]{figure/s/fare_eps1m50000p950_ell}
	}
	\subfigure[Distance, 0.95, 860, 1036]{
		\includegraphics[width=0.31\textwidth]{figure/s/dist_eps1m50000p950_ell}
	}
	
	\centering
	\subfigure[Time, 0.995, 2880, 3628]{
		\includegraphics[width=0.31\textwidth]{figure/s/time_eps1m50000p995_ell}
	}
	\subfigure[Fare, 0.995, 1839, 2037]{
		\includegraphics[width=0.31\textwidth]{figure/s/fare_eps1m50000p995_ell}
	}
	\subfigure[Distance, 0.995, 1839, 2037]{
		\includegraphics[width=0.31\textwidth]{figure/s/dist_eps1m50000p995_ell}
	}
	\caption{Empirical average error of percentile estimation. $\epsilon=0.1$.}
\end{figure*}


\begin{figure*}[ht]
	\centering
	\subfigure[Time, 0.85, 1411, 1295]{
		\includegraphics[width=0.31\textwidth]{figure/s/time_eps5m50000p850_ell}
	}
	\subfigure[Fare, 0.85, 525, 440]{
		\includegraphics[width=0.31\textwidth]{figure/s/fare_eps5m50000p850_ell}
	}
	\subfigure[Distance, 0.85, 525, 440]{
		\includegraphics[width=0.31\textwidth]{figure/s/dist_eps5m50000p850_ell}
	}
	
	\centering
	\subfigure[Time, 0.95, 1928, 1959]{
		\includegraphics[width=0.31\textwidth]{figure/s/time_eps5m50000p950_ell}
	}
	\subfigure[Fare, 0.95, 860, 1036]{
		\includegraphics[width=0.31\textwidth]{figure/s/fare_eps5m50000p950_ell}
	}
	\subfigure[Distance, 0.95, 860, 1036]{
		\includegraphics[width=0.31\textwidth]{figure/s/dist_eps5m50000p950_ell}
	}
	
	\centering
	\subfigure[Time, 0.995, 2880, 3628]{
		\includegraphics[width=0.31\textwidth]{figure/s/time_eps5m50000p995_ell}
	}
	\subfigure[Fare, 0.995, 1839, 2037]{
		\includegraphics[width=0.31\textwidth]{figure/s/fare_eps5m50000p995_ell}
	}
	\subfigure[Distance, 0.995, 1839, 2037]{
		\includegraphics[width=0.31\textwidth]{figure/s/dist_eps5m50000p995_ell}
	}
	\caption{Empirical average error of percentile estimation. $\epsilon=0.5$.}
\end{figure*}


\begin{figure*}[ht]
	\centering
	\subfigure[Time, 0.85, 1411, 1295]{
		\includegraphics[width=0.31\textwidth]{figure/s/time_eps10m50000p850_ell}
	}
	\subfigure[Fare, 0.85, 525, 440]{
		\includegraphics[width=0.31\textwidth]{figure/s/fare_eps10m50000p850_ell}
	}
	\subfigure[Distance, 0.85, 525, 440]{
		\includegraphics[width=0.31\textwidth]{figure/s/dist_eps10m50000p850_ell}
	}
	
	\centering
	\subfigure[Time, 0.95, 1928, 1959]{
		\includegraphics[width=0.31\textwidth]{figure/s/time_eps10m50000p950_ell}
	}
	\subfigure[Fare, 0.95, 860, 1036]{
		\includegraphics[width=0.31\textwidth]{figure/s/fare_eps10m50000p950_ell}
	}
	\subfigure[Distance, 0.95, 860, 1036]{
		\includegraphics[width=0.31\textwidth]{figure/s/dist_eps10m50000p950_ell}
	}
	
	\centering
	\subfigure[Time, 0.995, 2880, 3628]{
		\includegraphics[width=0.31\textwidth]{figure/s/time_eps10m50000p995_ell}
	}
	\subfigure[Fare, 0.995, 1839, 2037]{
		\includegraphics[width=0.31\textwidth]{figure/s/fare_eps10m50000p995_ell}
	}
	\subfigure[Distance, 0.995, 1839, 2037]{
		\includegraphics[width=0.31\textwidth]{figure/s/dist_eps10m50000p995_ell}
	}
	\caption{Empirical average error of percentile estimation. $\epsilon=1$.}
\end{figure*}

==> figure/old/transaction1_ell.tex <==
\begin{figure*}[ht]
	\centering
	\subfigure[kosarak, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/kosarak_eps1m50000p850_ell}
	}
	\subfigure[pos, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/pos_eps1m50000p850_ell}
	}
	\subfigure[retail, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/retail_eps1m50000p850_ell}
	}
	
	\centering
	\subfigure[kosarak, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/kosarak_eps1m50000p950_ell}
	}
	\subfigure[pos, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/pos_eps1m50000p950_ell}
	}
	\subfigure[retail, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/retail_eps1m50000p950_ell}
	}
	
	\centering
	\subfigure[kosarak, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/kosarak_eps1m50000p995_ell}
	}
	\subfigure[pos, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/pos_eps1m50000p995_ell}
	}
	\subfigure[retail, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/retail_eps1m50000p995_ell}
	}
	\caption{Empirical average error of percentile estimation. $\epsilon=0.1$.}
\end{figure*}


\begin{figure*}[ht]
	\centering
	\subfigure[kosarak, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/kosarak_eps5m50000p850_ell}
	}
	\subfigure[pos, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/pos_eps5m50000p850_ell}
	}
	\subfigure[retail, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/retail_eps5m50000p850_ell}
	}
	
	\centering
	\subfigure[kosarak, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/kosarak_eps5m50000p950_ell}
	}
	\subfigure[pos, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/pos_eps5m50000p950_ell}
	}
	\subfigure[retail, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/retail_eps5m50000p950_ell}
	}
	
	\centering
	\subfigure[kosarak, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/kosarak_eps5m50000p995_ell}
	}
	\subfigure[pos, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/pos_eps5m50000p995_ell}
	}
	\subfigure[retail, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/retail_eps5m50000p995_ell}
	}
	\caption{Empirical average error of percentile estimation. $\epsilon=0.5$.}
\end{figure*}


\begin{figure*}[ht]
	\centering
	\subfigure[kosarak, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/kosarak_eps10m50000p850_ell}
	}
	\subfigure[pos, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/pos_eps10m50000p850_ell}
	}
	\subfigure[retail, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/retail_eps10m50000p850_ell}
	}
	
	\centering
	\subfigure[kosarak, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/kosarak_eps10m50000p950_ell}
	}
	\subfigure[pos, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/pos_eps10m50000p950_ell}
	}
	\subfigure[retail, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/retail_eps10m50000p950_ell}
	}
	
	\centering
	\subfigure[kosarak, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/kosarak_eps10m50000p995_ell}
	}
	\subfigure[pos, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/pos_eps10m50000p995_ell}
	}
	\subfigure[retail, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/retail_eps10m50000p995_ell}
	}
	\caption{Empirical average error of percentile estimation. $\epsilon=1$.}
\end{figure*}

==> figure/old/transaction2_ell.tex <==
\begin{figure*}[ht]
	\centering
	\subfigure[web1, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/web1_eps1m50000p850_ell}
	}
	\subfigure[web2, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/web2_eps1m50000p850_ell}
	}
	\subfigure[star, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/star_eps1m50000p850_ell}
	}
	
	\centering
	\subfigure[web1, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/web1_eps1m50000p950_ell}
	}
	\subfigure[web2, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/web2_eps1m50000p950_ell}
	}
	\subfigure[star, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/star_eps1m50000p950_ell}
	}
	
	\centering
	\subfigure[web1, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/web1_eps1m50000p995_ell}
	}
	\subfigure[web2, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/web2_eps1m50000p995_ell}
	}
	\subfigure[star, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/star_eps1m50000p995_ell}
	}
	\caption{Empirical average error of percentile estimation.   $\epsilon=0.1$.}
\end{figure*}


\begin{figure*}[ht]
	\centering
	\subfigure[web1, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/web1_eps5m50000p850_ell}
	}
	\subfigure[web2, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/web2_eps5m50000p850_ell}
	}
	\subfigure[star, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/star_eps5m50000p850_ell}
	}
	
	\centering
	\subfigure[web1, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/web1_eps5m50000p950_ell}
	}
	\subfigure[web2, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/web2_eps5m50000p950_ell}
	}
	\subfigure[star, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/star_eps5m50000p950_ell}
	}
	
	\centering
	\subfigure[web1, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/web1_eps5m50000p995_ell}
	}
	\subfigure[web2, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/web2_eps5m50000p995_ell}
	}
	\subfigure[star, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/star_eps5m50000p995_ell}
	}
	\caption{Empirical average error of percentile estimation.   $\epsilon=0.5$.}
\end{figure*}


\begin{figure*}[ht]
	\centering
	\subfigure[web1, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/web1_eps10m50000p850_ell}
	}
	\subfigure[web2, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/web2_eps10m50000p850_ell}
	}
	\subfigure[star, 0.85]{
		\includegraphics[width=0.31\textwidth]{figure/s/star_eps10m50000p850_ell}
	}
	
	\centering
	\subfigure[web1, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/web1_eps10m50000p950_ell}
	}
	\subfigure[web2, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/web2_eps10m50000p950_ell}
	}
	\subfigure[star, 0.95]{
		\includegraphics[width=0.31\textwidth]{figure/s/star_eps10m50000p950_ell}
	}
	
	\centering
	\subfigure[web1, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/web1_eps10m50000p995_ell}
	}
	\subfigure[web2, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/web2_eps10m50000p995_ell}
	}
	\subfigure[star, 0.995]{
		\includegraphics[width=0.31\textwidth]{figure/s/star_eps10m50000p995_ell}
	}
	\caption{Empirical average error of percentile estimation.   $\epsilon=1$.}
\end{figure*}




==> old/app_update_thres.tex <==
\section{Different Ways of Updating $\tau$}
\label{app:update_thres}
We decompose the problem of updating $\tau$ into three sub-problems: (1) decide when to update; (2) which direction should we change $\tau$; and (3) how much is the change.  We first analyze the general problem of {\it deciding above or below}.




\mypara{Above or Below}
We want to decide whether the desired threshold is above or below the old threshold.  There are two methods to do it: (1) using Laplace mechanism to publish the value, and then compare the noisy value with the threshold; and (2) using EM to output either above or below.  Intuitively, the second technique may be better because it gives the minimal information (only one bit).  To formally compare the two methods, we calculate the probability the correct answer is generated.  Suppose the private value is $t$, and the threshold is $T$, we have:
In LM, the output is $t+\eta$ where $\eta = \Lapp{\frac{1}{\epsilon}}$ (sensitivity is $1$).  Given $t>T$ (denote $b=t-T$), 
\begin{align}
    \Pr{t+\eta > T} = \Pr{\eta > T - t} = 1 - \Pr{\eta < T - t} =  \frac{1}{2}\exp{\left(-(T-t)\epsilon\right)} =  \frac{1}{2}\exp{\left(b\epsilon\right)}\label{eq:lm_correct_prob}
\end{align}

% As $\Pr{\Lapp{\frac{1}{\epsilon}}=x}  = \frac{1}{2\beta} \myexp{-|x|\epsilon}$
    
    
For EM, we define the quality function for outputting $+1$ or $-1$ as
\begin{align*}
    q_{+1}(D) = t - T \\
    q_{-1}(D) = T - t
\end{align*} 

This gives the probability of outputting $+1$ to be
\begin{align}
     \Pr{\AA_q(t)=+1} = \frac{\exp{\left(\frac{\epsilon b }{2}\right)}}{\exp{\left(\frac{\epsilon b}{2}\right)} + \exp{\left(\frac{-\epsilon b}{2}\right)}} = \frac{\exp{\left(\epsilon b\right)}}{\exp{\left(\epsilon b\right)} + 1}\label{eq:em_correct_prob}
\end{align}
Comparing Equation~\eqref{eq:lm_correct_prob} with Equation~\eqref{eq:em_correct_prob}, we have \eqref{eq:lm_correct_prob} is always greater than \eqref{eq:em_correct_prob} because $\exp{\left(b\epsilon\right)} > 1$.  Note that even if the quality functions in EM are monotonic, this still holds.  Thus Laplace mechanism always performs better.
Moreover, we can extend the method with a ``buffer''.  That is, if $t$ is close to $T$, we allow the output of $0$.


\begin{algorithm}[!htb]
	\caption{Find how to update $\ell$}\label{algo:svt_tau_bi}
	\begin{algorithmic}[1]
		\Function{UpdateLimit}{$V, \epsilon, \tau$} 
    		\State $\epsilon_1 \gets \frac{\epsilon}{2}, \epsilon_2 \gets \frac{\epsilon}{2}, \mathsf{GS}_q \gets 1$
    		\State $\rho \gets \Lapp{\frac{\mathsf{GS}_q}{\epsilon_1}}$
    		\For {$i = 1$ to $+\infty$}
		        \State $q_{i,1}(V) \gets p \cdot |V| - |\{j\mid v_j \le \ell_m - (i - 1) \}|$
		        \If {$q_{i,1}(V) + \Lapp{\frac{2\mathsf{GS}_q}{\epsilon_2}} \ge \rho$}
                    \State \Return $i,1$
                \EndIf
		        \State $q_{i,2}(V) \gets |\{j\mid v_j \le i \}| - p \cdot |V|$
                \If {$q_{i,2}(V) + \Lapp{\frac{2\mathsf{GS}_q}{\epsilon_2}} \ge \rho$}
                    \State \Return $i,2$
                \EndIf
    		\EndFor
	    \EndFunction
	\end{algorithmic}
\end{algorithm}


\mypara{How Much to Change}
Having decided whether to go up or down, we can then decide how much change we want to apply to $\tau$.  Setting a pre-defined change quantity helps when the change is predictable, but when the data change drastically, using SVT to obtain it seems more reasonable.  Note that it is also possible to decide the new $\tau$ (both direction and step) at once.  We thus have the following options:
\begin{itemize}
    \item Algorithm~\ref{algo:svt_tau}.  Note that this does not utilize the information of the last $\tau$.
    \item Using SVT but searching for two directions, starting from $1$ and $\ell_m$.  In particular, we define the sequence of queries
    \begin{align*}
        q_{i,1}(V) &=  p \cdot |V| - |\{j\mid v_j \le \ell_m - (i - 1)\}| , \\
        q_{i,2}(V) &= |\{j\mid v_j \le i\}| - p \cdot |V| .
    \end{align*}
    Algorithm~\ref{algo:svt_tau_bi} gives the full procedure.  Note that the queries are no longer monotonic.   
    % Although this utilizes the last $\tau$, this may not help, as the current $\tau$ may be far from the previous $\tau$.  In some cases, this gives worse result than the naive Algorithm~\ref{algo:svt_tau} (e.g., when the current $\tau$ is small and the previous $\tau$ is large).  
    \item First decide whether the desired $\tau$ is above or below the currently used $\tau$, and then use SVT but searching with only one direction from $\tau$.  That is,
    \begin{align*}
        q_i(V) &=  p \cdot |V| - |\{j\mid v_j \le \tau - i\}| &\mbox{ if we want to decrease}, \\
        q_i(V) &= |\{j\mid v_j \le \tau + i\}| - p \cdot |V| &\mbox{ if we want to increase}.
    \end{align*}
\end{itemize}

Compared to the third option, the second option searches in one wrong direction, note that the third option also spend some privacy budget in determining the direction.  Which method is better actually depends on the underlying data.  Intuitively, if the desired $\tau$ is larger than the previous $\tau$, method (3) trades-off some privacy budget to save the initial searches.  If on the other hand, it is smaller and closer to the starting point, method (1) will be better.


\mypara{When to Update}
% Given the technique to test whether the threshold is set too high or too low, we then investigate when should this test be used, how frequent it should be used.
We can always update  $\tau$ periodically.  On the other hand, we can also decide whether or not to update based on the observed noisy counts.  For example, one heuristic could be to test whether the mean of the noisy counts is close to the threshold.  What is more interesting is to use SVT for this test.  In particular, at each observation, we test whether we should change $\tau$.  Here we use a threshold $\theta$; and if the desired $\tau$ deviates from the previous one by more than $\theta$, we want to update it.  There are several variants we can consider:


\begin{itemize}
    \item Testing whether the $\tau$ so far deviates from the previous one by a large amount.  In particular, define the sequence of queries
    \begin{align*}
        q_i(V) &= \max(|\{j\mid v_j\le \tau, j \le i\}| - p i, 0) - \theta i
    \end{align*}
    Note that each query takes a prefix of the observations $v_1$ till $v_i$, while previous discussions focus on fixing the observations.  The procedure is presented in Algorithm~\ref{algo:svt_tau_update}.  
    
    \item Detect both when to update $\tau$ and the direction (above or below) together.  That is, define the sequence of queries
    \begin{align*}
        q_{i,1}(V) &= |\{j\mid v_j \le \tau, j \le i\}| - (p+\theta) i, \\
        q_{i,2}(V) &= (p-\theta) i - |\{j\mid v_j \le \tau, j \le i\}|.
    \end{align*}
    The procedure is presented in Algorithm~\ref{algo:svt_tau_update_bi}.  
    
    \item Finally, we can detect when, which direction, and how much to change $\tau$ in one SVT.  The idea is to extend each query of Algorithm~\ref{algo:svt_tau_update_bi} with a sequence of queries (from the idea of Algorithm~\ref{algo:svt_tau_bi}).  In particular,
    \begin{align*}
        q_{i,1,j}(V) &= |\{k\mid v_k \le \min(j,\tau), k \le i\}| - (p+\theta) i, \\
        q_{i,2,j}(V) &= (p-\theta) i - |\{k\mid v_k \le \max(\ell_m+1-j,\tau), k \le i\}|.
    \end{align*}
\end{itemize}
After the algorithm returns, one can resume it with the rest of the observations.

Overall, it is desired to start warm, because we have to use the threshold up front, and without sufficient observations, it cannot be reliably determined.  That is, we may update more frequently from the beginning, and less frequently later.

How many observations we use for this test is another aspect to consider.  Intuitively, the more data, the better the result will be.  However, some data may be obsolete and thus influence with the result. 



\begin{algorithm}[!htb]
	\caption{Find when to update $\tau$}\label{algo:svt_tau_update}
	\begin{algorithmic}[1]
		\Function{UpdateLimit}{$V, \epsilon, \tau$} 
    		\State $\epsilon_1 \gets \frac{\epsilon}{2}, \epsilon_2 \gets \frac{\epsilon}{2}, \mathsf{GS}_q \gets 1$
    		\State $\rho \gets \Lapp{\frac{\mathsf{GS}_q}{\epsilon_1}}$
    		\For {$i = 1$ to $+\infty$}
		        \State $q_i(V) \gets \max(|\{j\mid v_j\le \tau, j \le i\}| - p i, 0) - \theta i$
                \If {$q_i(V) + \Lapp{\frac{2\mathsf{GS}_q}{\epsilon_2}} \ge \rho$}
                    \State \Return $i$
                \EndIf
    		\EndFor
	    \EndFunction
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}[!htb]
	\caption{Find when and how to update $\ell$}\label{algo:svt_tau_update_bi}
	\begin{algorithmic}[1]
		\Function{UpdateLimit}{$V, \epsilon, \tau$} 
    		\State $\epsilon_1 \gets \frac{\epsilon}{2}, \epsilon_2 \gets \frac{\epsilon}{2}, \mathsf{GS}_q \gets 1$
    		\State $\rho \gets \Lapp{\frac{\mathsf{GS}_q}{\epsilon_1}}$
    		\For {$i = 1$ to $+\infty$}
		        \State $q_{i,1}(V) \gets|\{j\mid v_j \le \tau, j \le i\}| - (p+\theta) i$
                \If {$q_{i,1}(V) + \Lapp{\frac{2\mathsf{GS}_q}{\epsilon_2}} \ge \rho$}
                    \State \Return $i,1$
                \EndIf
		        \State $q_{i,2}(V) \gets (p-\theta) i - |\{j\mid v_j \le \tau, j \le i\}|$
                \If {$q_{i,2}(V) + \Lapp{\frac{2\mathsf{GS}_q}{\epsilon_2}} \ge \rho$}
                    \State \Return $i,2$
                \EndIf
    		\EndFor
	    \EndFunction
	\end{algorithmic}
\end{algorithm}

==> old/percentile_analysis.tex <==
\subsection{What Percentile}
Before presenting the method to estimate the percentile, we first analyze what percentile is appropriate.  We consider the accuracy of estimating each value, measured by the mean squared error.  That is, assume $v'$ is the estimation of $v$.  We have:
\begin{align*}
    \EV{(v'-v)^2} 
    =& \EV{v'^2-2vv'+v^2}\\
    =& \EV{v'^2}-2v\EV{v'}+v^2\\
    =& \EV{v'^2} - \EV{v'}^2 + \EV{v'}^2-2v\EV{v'}+v^2\\
    =& \left(\EV{v'^2} - \EV{v'}^2\right) + \left(\EV{v'} - v\right)^2\\
    =& \Var{v'} + \Bias{v'}^2
\end{align*}
It is composed of two parts: variance of $v'$ and the squared bias of $v'$.  

In our case, $v'$ is computed by the Laplace mechanism with privacy budget $\epsilon$ and sensitivity $2\tau$.  The variance of $v'$ is $8\frac{\tau^2}{\epsilon^2}$.  For the bias, it is introduced by truncation to $\tau$.  Thus for any value $v>\tau$, the bias $\Bias{v'}=v-\tau$.  Now we calculate $\Bias{v'}$.  We assume the values follow an exponential distribution.  That is, for any value $v$, $\Pr{v=\ell} = \frac{1}{\lambda}e^{-\lambda\ell}$, and $\Pr{v<\ell} = e^{-\lambda\ell}$.  This is the assumption made in~\cite{ndss:perrier2019private} and we also verified this in the dataset we use in the experiment.  Then 
\begin{align*}
    \Bias{v'} =& \int_\tau^\infty \Pr{v}(v-\tau)dv\\
    =&\int_\tau^\infty \lambda v e^{-\lambda v}dv - \tau \int_\tau^\infty \lambda e^{-\lambda v}dv\\
    =&\left(\tau + \frac{1}{\lambda}\right)e^{-\lambda\tau} -\tau e^{-\lambda\tau}\\
    =&\frac{e^{-\lambda\tau}}{\lambda} 
\end{align*}

\begin{align*}
    \frac{\partial \mse}{\partial \tau} =& \frac{\partial \left(\Var{v} + \Bias{v}^2\right)}{\partial \tau}\\
    =& \frac{\partial \left(8\frac{\tau^2}{\epsilon^2} + \frac{e^{-2\lambda\tau}}{\lambda^2}\right) }{\partial \tau}\\
    =& \frac{16\tau}{\epsilon^2} - \frac{2}{\lambda}e^{-2\lambda\tau} = 0\\    
    \implies& \tau e^{-2\lambda\tau} = \frac{\epsilon^2}{8\lambda}
\end{align*}

==> old/primitive_svt.tex <==

\mypara{Sparse Vector Technique}
The Sparse Vector Technique (SVT)~\cite{stoc:dwork2009complexity} can output some query answers without costing any privacy budget.  Given a (possibly infinite) sequence of queries $q_1, q_2, \ldots$, SVT outputs a vector indicating whether each query answer is positive or not.  
More specifically, define the sensitivity 
$$ \mathsf{GS}_q = \max_{i} \max_{V\simeq V'} |q_i(V) - q_i(V')|. $$
SVT works by first drawing a Laplace noise $\rho = \Lapp{\frac{\mathsf{GS}_q}{\epsilon_1}}$ and then comparing each query answer (individually perturbed by Laplace mechanism with $\Lapp{\frac{2c\mathsf{GS}_q}{\epsilon_2}}$) against $\rho$, where $c$ is the desired number of indices whose positive answers are positive.  The privacy budget is consumed only when the noisy answer is above $\rho$.  After encountering $c$ positive answers, SVT terminates.  
Similar to the Exponential Mechanism, if the queries satisfy the monotonic condition, i.e., $
\forall_{V\simeq V'}$,
\[
\left(\exists_{i}\, q_i(V) \!<\! q_i(V')\right) \!\rightarrow\! \left(\forall_{j}\,q_j(V) \!\leq \! q_j(V')\right)
\]
then one can remove the factor of $2$ and use $\Lapp{\frac{c\mathsf{GS}_q}{\epsilon_2}}$ to perturb each query answer.


The SVT technique was first proposed in~\cite{stoc:dwork2009complexity} by Dwork et al.  In~\cite{pvldb:lyu2017understanding}, Lyu et al. analyzed and identified pitfalls of SVT implementations, and proposed an SVT that optimizes privacy budget allocation.  It was also pointed out in~\cite{pvldb:lyu2017understanding} that the SVT technique is unnecessary in non-interactive setting, and can be replaced by the Exponential Mechanism with better accuracy. In this paper we show that this statement is not always true when SVT can enjoy the monotonic property. 

==> old/sec_analysis.tex <==
\section{Theoretical Analysis of the Methods}
In some cases, it is unnecessary to use hierarchical methods.

\pgs uses some flavor of the DAWA method. 
Here as we apply the hierarchical method, we cannot adaptively choose the branching factor.  This is because one has to have a global view of the whole dataset in order to adaptively branch.  But the setting is sequential.  One has to output information before having the global view.



==> old/svt_percentile.tex <==

% In what follows, we first consider the task of outputting a target percentile under DP.  Given a percent rank $p$, a $p$-th percentile is a measure used in statistics indicating the value below which $p$ percent of samples falls.   This task is also considered in \pak.  While \pak proposes to use a modified version of smooth sensitivity, we propose to use the sparse vector technique (SVT).  We notice that this result is of independent interest and can be applied to settings that need percentiles.  

% Note that there are two natural alternatives: using Exponential Mechanism, or calculating it from the noisy histograms from Laplace Mechanism.  We realize that using the SVT technique one can get much better accuracy.


\begin{comment}
\subsection{Existing Work for Percentiles}
Besides \pak~\cite{ndss:perrier2019private}, there are other methods that can output the percentile.  In particular, \cite{sigmod:tao20localsensitivity} provides DP SQL engines for multiple tables.  The sensitivity of the tables can be unbounded (each user may contribute multiple records to the tables).  To limit the contribution, which is closely related to sensitivity, it uses SVT to find a threshold.  
\begin{align*}
    q_i(V) = \frac{Q_i(V) - \hat{Q}_{\ell_{\max}}(V)}{i}
\end{align*}
where $Q_i(V)$ is the query result on $V$ after truncating values to $i$ (the original method uses ``removing''; but we believe truncation is more suitable in our case).  In our setting, $Q$ can be a random range query.  $\hat{Q}$ is the noisy result by applying $\epsilon/10$ as privacy budget (and SVT uses $9/10$ of the privacy budget). \says{tianhao}{the method may not apply here}


In~\cite{asiaccs:day2015differentially}, EM algorithm is used.  Although the settings are different, the methods are general and can be used in our setting.  
\begin{align*}
    q_i(V) = \frac{1}{n}\sum_{j}v_j - \frac{i}{\epsilon}
\end{align*}
\end{comment}

\subsubsection{Baseline: Using EM for Percentiles}
\label{subsec:em_percentile}
Our goal is to output the $p$-th percentile from a candidate set.  This problem is the motivation of introducing the exponential mechanism (EM).  Thus as a warm starter, we first consider using EM to solve the problem.  To design an EM algorithm, a key technical challenge is to come up with a sequence of low-sensitivity query functions that can measure the desirability of choosing a particular percentile.  A good choice makes the desired result returned with high confidence.

Denote $m$ as the number of observations to be used in EM, and $m_i$ as the number of values from these $m$ observations that are smaller than $i$, i.e., $m_i=|\{j\mid v_j \le i, j\in[m] \}|$ where $[x]=\{1,2,\ldots,x\}$ and $|X|$ denotes the cardinality of set $X$. We define the quality function $i$ as the following:
% negative value of the absolute difference between the target amount of values $pm$ and the number of values that are smaller than $i$: 
\begin{align}
    q_i(V) = -| p m - m_i |\label{eq:em_q}
\end{align} 
This ensures the target $\theta$ has the highest score, and the sensitivity is $1$. 
We then draw the threshold using EM given in Equation~\ref{eq:exp}.  
In Figure~\ref{fig:emcdf}, we plot the quality scores for two target percentile ranks (denoted by the two horizontal dashed lines).  Note that to make the scores fit in the CDF figure, we add $pm$ to each score and then divide it by $m$.  
% The new quality function gives equivalent result as that in Equation~\ref{eq:em_q}, because the factor of $pm$ cancels out when we use EM in Equation~\ref{eq:exp}.  
We can see that when $p$ is small (the lower line), the score of the target has a clear advantage over others.  However, when $p$ is larger, the advantage diminished and it is more likely that a very large $\theta$ is selected.  To overcome this issue, we propose a new method using SVT.

% \begin{algorithm}[!htb]
% 	\caption{EM-P: Find the $p$-th percentile using EM. }\label{algo:svt_tau}
% 	\begin{algorithmic}[1]
% 		\Function{SVT-P}{$V, \epsilon, p, B$} 
%     		\State $m\gets |V|, \mathsf{GS}_q \gets 1$ %\Comment{Sensitivity is 1}
%     		\State $\rho \gets \Lapp{\frac{\mathsf{GS}_q}{\epsilon_1}}$
%     		\For {$i = 1$ to $B$}
%                 \State $m_i \gets |\{i\mid v_i \le i\}|$
%                 \If {$m_i - pm + \Lapp{\frac{\mathsf{GS}_q}{\epsilon_2}}\ge \rho$}
%                     \State \Return $\ell$
%                 \EndIf
%     		\EndFor
% 	    \EndFunction
% 	\end{algorithmic}
% \end{algorithm}

\begin{figure}[t]
    \centering
    \includegraphics[width = 0.46\textwidth]{figure/emcdf.eps}
    \caption{The blue curve is the CDF of the distribution.  When EM is used, scores above the horizontal lines are reflected (by taking the absolute value of Equation~\ref{eq:em_q}).  Comparing to $\tau_1$, there are more candidates with similar quality scores around $\tau_2$, which makes it likely to select a higher threshold.}
    \label{fig:emcdf}
\end{figure}{}



\subsubsection{Improved: Using SVT for Percentiles}
\label{subsec:svt_percentile}
SVT is used to find the first $k$ queries whose answers are positive.  In our case, $k=1$ because we only need one percentile.
% Note that a equivalent version is to associate each query with a threshold, so that SVT outputs the first $k$ queries whose answers are above the given thresholds.  
% As the threshold can be put into the query function, by subtracting the desired threshold, it is equivalent to test whether the query result is above zero.
%  (in our case, the query answer is high above $0$).  
% If not, we want a result that is nearly as desired, rather than a very undesired result.  
% That is, the query answer reflects our preference.
% \mypara{SVT for Percentiles}
For the problem of estimating percentiles, we define query $i$ as:
% the number of records smaller than $i$ minus $pm$, i.e., 
\begin{align}
    q_i(V) = m_i - p \cdot m\label{eq:svt_q}
\end{align} 
Compared to the quality function given in Equation~\ref{eq:em_q}, this removes the absolute operation because we only need the first index whose query result (or quality score) is above $0$.  The sensitivity of the quality function is $1$.  Moreover, the queries are monotonic (see the CDF of Figure~\ref{fig:emcdf}).
% \begin{fact}
% The quality function in Equation~\ref{eq:svt_q} is monotonic:
% \[
% \left(\exists_{i}\, q_{i}(V) \!<\! q_{i}(V')\right) \!\implies\! \left(\forall_{j}\,q_{j}(V) \!\leq \! q_{j}(V')\right)
% \]
% \end{fact}
Algorithm~\ref{algo:svt_tau} gives the details of the method.  
We set $\epsilon_1 = \epsilon_2 = \epsilon / 2$ according to the guidance from~\cite{pvldb:QardajiYL13}.
% \begin{figure}[!h]
%     \centering
%     \includegraphics[width = 0.46\textwidth]{figure/svtcdf.eps}
%     \caption{While estimating percentile, SVT gives decent accuracy at low threshold where a steep slope can be found, such as $\tau_1$ in this figure. On the other hand, it performs less reliably around higher threshold.}
%     \label{fig:svtcdf}
% \end{figure}{}

\begin{algorithm}[!htb]
	\caption{SVT-P: Find the $p$-th percentile using SVT.  Note that $V$ is the first $m$ observations.}\label{algo:svt_tau}
	\begin{algorithmic}[1]
		\Function{SVT-P}{$V, \epsilon, p, B$} 
    		\State $m\gets |V|, \epsilon_1 \gets \frac{\epsilon}{2}, \epsilon_2 \gets \frac{\epsilon}{2}, \mathsf{GS}_q \gets 1$ %\Comment{Sensitivity is 1}
    		\State $\rho \gets \Lapp{\frac{\mathsf{GS}_q}{\epsilon_1}}$
    		\For {$i = 1$ to $B$}
                \State $m_i \gets |\{i\mid v_i \le i, i\in[m]\}|$
                \If {$m_i - pm + \Lapp{\frac{\mathsf{GS}_q}{\epsilon_2}}\ge \rho$}
                    \State \Return $\ell$
                \EndIf
    		\EndFor
	    \EndFunction
	\end{algorithmic}
\end{algorithm}


There are several observations of this SVT algorithm.  The first one is that the order of the queries also carry preferences from the user.  That is, for any two queries with the same answer, the former one always has a higher probability of being returned than the latter.
% because SVT could abort after returning the formal query, and the latter will never be returned.   
\begin{observation}
For two queries $q_i$ and $q_j$ with $i<j$ and $q_i=q_j$, the probability the first query is returned is higher than that of the second, namely, $\Pr{i\gets\mbox{SVT} }>\Pr{j\gets\mbox{SVT} }$.
\end{observation}
This is because if we look at them independently, the probabilities of being returned are the same.  However, the event that the second query is returned is conditioned on the event that the first query is not returned.  This also implies that SVT tends to introduce a negative bias to the result.  
% If we have a choice of ordering is to put preferable queries up front.
% But because of the noise incurred by DP, the ideal case may not be achieved and we may end up with queries whose answers are below the threshold, or we miss some of the first queries.  These cases may not be vital in some settings, e.g., when the query answer reflects our preference of choosing the query.  But in the setting considered in this paper, where the goal is to find the $\tau$ s.t., $p\%$ of the values are less than it, this can give greater errors.  

Moreover, if we put Equation~\ref{eq:svt_q} into Figure~\ref{fig:emcdf}, the blue curve is the cumulative density (the first term of the equation) and is not reflected.  When it is above the percent rank $p$, indicated by the horizontal dashed lines, Algorithm~\ref{algo:svt_tau} will return (of course due to the DP noise, both the horizontal lines and the CDF curve will be perturbed a little bit).  If $p$ corresponds to the lower green line, values before the desired $\theta_1$ have much smaller probabilities of being returned.  
On the other hand, if $p$ corresponds to the higher orange line, values before the desired $\theta_2$ have noticeable probabilities of being returned.  If there are many such values (meaning that the curve is flattened before $\theta_2$), the result will include a large negative bias.  This effect is summarized as follows in Observation~\ref{obs:svt_bias}.  
% We will provide solution to avoid this effect in Section~\ref{subsec:em_threshold}.  
\begin{observation}
\label{obs:svt_bias}
Algorithm~\ref{algo:svt_tau} performs well when the queries before the target has much lower scores, but poorly when they have very close scores.
\end{observation}

% \input{old/percentile_analysis}

% Comparing EM and SVT in Figure~\ref{fig:emcdf}, EM tends to select larger thresholds while SVT tends to select smaller ones.  
Another thing we want to highlight is the choice between SVT and EM.  In~\cite{pvldb:lyu2017understanding}, the authors state that in the non-adaptive setting (the queries are fixed and not dependent on the previous result), using EM can always give better result than SVT. 
Here we amend this statement by introducing a special case that when the queries in EM can be converted to a monotonic sequence like the one shown Figure~\ref{fig:emcdf}, SVT is more preferable, as we will empirically show in Section~\ref{sec:exp}. 
% One key thing that makes SVT preferable is that the quality function in SVT is monotonic.  

% Here we clarify this statement by differentiating two cases of using EM/SVT:  The first is to select the queries with the highest scores; in this setting EM is more preferable to SVT.  This is also the assumption in~\cite{pvldb:lyu2017understanding}.  The second is case is to select the first few queries whose scores are above a threshold (instead of highest).  And in this case, SVT can actually give better result.
% \begin{observation}
% When queries are sorted by scores and the goal is to return the first few queries above a threshold, SVT gives better result than EM.
% \end{observation}

% \mypara{On Step Size}
% By default, we work on the finest granularity (e.g., 1).  It is possible to vary the step size.  The intuition is that, with larger step sizes, one may pass through the target, but one is less prone to select a value below the target (because the sample rate is smaller).  This is also the case for the Exponential Mechanism.

% \mypara{On Budget Partition}
% \cite{pvldb:QardajiYL13} suggests setting $\epsilon_1 = \epsilon_2 = \epsilon / 2$.  With different step sizes, it might be possible to choose different partitioning to have better utility.

==> old/utility.tex <==

% \subsection{Utility Metrics}


% \mypara{Quantiles}
% Quantiles are cut points dividing the range of a probability distribution into intervals with equal probabilities.  Formally, $\mathbf{Q}(\x, \beta) = \arg\max_v\{F(\x, v) \leq \beta \}$.
% In the experiment, define $B = \{ 10\%, 20\%, \ldots, 90\%\}$, we measure the following 
% \begin{align*}
%     \frac{1}{|B|}\sum_{\beta\in B}|\mathbf{Q}(\x, \beta) - \mathbf{Q}(\estx, \beta)|
% \end{align*}




% \mypara{Kolmogorov-Smirnov distance (KS-distance)}
% KS-distance is the maximum absolute difference at any point between estaimated and true CDF.  The KS-distance $d_{KS}$ can be express as
%     \begin{align*}
%         d_{KS}(V_c, \tilde{V}_c) = \sup_{v\in \Domain}|V_c(v) - \tilde{V}_c(v)|
%     \end{align*}

% The ultimate goal is to obtain a differentially private stream $\tilde{V}$ that is close to $V$.  
Following the setting of~\cite{ndss:perrier2019private}, the first $m$ readings are reserved for pre-processing (finding the threshold in~\cite{ndss:perrier2019private}).
For the rest of them, we measure the similarity between the private stream and the estimated stream using range queries, similar to~\cite{ndss:perrier2019private}.  Specifically, define $V(i, j)$ as the sum of the stream from index $i$ to $j$, i.e., $V(i, j) = \sum_{k=i}^j v_k$.  The metric is the expected squared error of any randomly sampled range query
\begin{align}
    \EV{\left(\tilde{V}(i, j) - V(i, j)\right)^2}\label{eq:ana_metric}
\end{align}

% Sum query as emphasized in~\cite{ndss:perrier2019private} is a special case of range query where $i=1$.

\begin{comment}
\subsubsection{Earth Mover Distance}
% We want the recovered density distribution to be as close to the true distribution.  However, since the distribution is over a metric space, we do not want to use purely point-wise distance metrics such as the $L_1$ and $L_2$ distance or the Kullback–Leibler (KL) divergence. To give a trivial example, if the ordinal domain is $\Domain = \{1,2,3,4\}$ and the true distribution on the domain is $\x = [0.7, 0.1, 0.1, 0.1]$, the two estimation $\estx_1 = [0.1, 0.7, 0.1, 0.1]$ and $\estx_2 = [0.1, 0.1, 0.1, 0.7]$ have the same $L_2$ distance from $\x$, but $\estx_1$ should be closer to $\x$ when we consider the ordinal nature.  Thus, in order to reflect the closeness between the estimation and the truth, we use two of the most popular distribution distances as metrics in our paper.
The error measure is an important aspect of the problem as we would like to quantify the ``distance'' between the original and the estimated distributions.  Ideally, we would like to measure this distance as the minimum number that must be added or removed from $V$ to get $\tilde{V}$.  
The standard error measures of Manhattan distance $||V- \tilde{V}||_1$ or sum-squared error $||V- \tilde{V}||_2$ do not capture this distance measure.  To see why, suppose $V = [0, 100, 0,
0, 0, 0]$. Consider two estimates $\tilde{V}_1 = [0, 0, 100, 0, 0, 0, 0]$ and $\tilde{V}_2 = [0, 0, 0, 0, 0, 100]$.  We see that $||V - \tilde{V}_1||_1 = ||V - \tilde{V}_2||_1 = 200$ and $||V - \tilde{V}_1||_2^2 = ||V - \tilde{V}_2||_2^2 = 20, 000$.  However, we should consider $\tilde{V}_1$ to be closer to $V$ than $\tilde{V}_2$ is.  

Thus, the appropriate way to measure distance between $V$ and $\tilde{V}$ is the Earthmover’s distance (emd) as it precisely captures the number that must be added to or removed from groups in $V$ in order to obtain $\tilde{V}$.  Normally, computing emd is not linear in the size of an array~\cite{ijcv:rubner2000earth}.  However, it can be computed in linear time for our problem by using the cumulative histograms.

\begin{lemma}[\cite{icde:li2007t}]
The earthmover’s distance between $V$ and $\tilde{V}$ can be computed as \begin{align*}
    \sum_{j=1}^n|\tilde{V}(1, j) - V(1, j)|.
\end{align*}
% $||C - \tilde{C}||_1$, where $C$ is the cumulative histogram of $V$, i.e., $c_i=\sum_{k=1}^i v_k$.
\end{lemma}
\end{comment}



==> percentile_analysis.tex <==
\subsection{What Percentile}
Before presenting the method to estimate the percentile, we first analyze what percentile is appropriate.  We consider the accuracy of estimating each value, measured by the mean squared error.  That is, assume $v'$ is the estimation of $v$.  We have:
\begin{align*}
    \EV{(v'-v)^2} 
    =& \EV{v'^2-2vv'+v^2}\\
    =& \EV{v'^2}-2v\EV{v'}+v^2\\
    =& \EV{v'^2} - \EV{v'}^2 + \EV{v'}^2-2v\EV{v'}+v^2\\
    =& \left(\EV{v'^2} - \EV{v'}^2\right) + \left(\EV{v'} - v\right)^2\\
    =& \Var{v'} + \Bias{v'}^2
\end{align*}
It is composed of two parts: variance of $v'$ and the squared bias of $v'$.  

In our case, $v'$ is computed by the Laplace mechanism with privacy budget $\epsilon$ and sensitivity $2\tau$.  The variance of $v'$ is $8\frac{\tau^2}{\epsilon^2}$.  For the bias, it is introduced by truncation to $\tau$.  Thus for any value $v>\tau$, the bias $\Bias{v'}=v-\tau$.  Now we calculate $\Bias{v'}$.  We assume the values follow an exponential distribution.  That is, for any value $v$, $\Pr{v=\ell} = \frac{1}{\lambda}e^{-\lambda\ell}$, and $\Pr{v<\ell} = e^{-\lambda\ell}$.  This is the assumption made in~\cite{ndss:perrier2019private} and we also verified this in the dataset we use in the experiment.  Then 
\begin{align*}
    \Bias{v'} =& \int_\tau^\infty \Pr{v}(v-\tau)dv\\
    =&\int_\tau^\infty \lambda v e^{-\lambda v}dv - \tau \int_\tau^\infty \lambda e^{-\lambda v}dv\\
    =&\left(\tau + \frac{1}{\lambda}\right)e^{-\lambda\tau} -\tau e^{-\lambda\tau}\\
    =&\frac{e^{-\lambda\tau}}{\lambda} 
\end{align*}

\begin{align*}
    \frac{\partial \mse}{\partial \tau} =& \frac{\partial \left(\Var{v} + \Bias{v}^2\right)}{\partial \tau}\\
    =& \frac{\partial \left(8\frac{\tau^2}{\epsilon^2} + \frac{e^{-2\lambda\tau}}{\lambda^2}\right) }{\partial \tau}\\
    =& \frac{16\tau}{\epsilon^2} - \frac{2}{\lambda}e^{-2\lambda\tau} = 0\\    
    \implies& \tau e^{-2\lambda\tau} = \frac{\epsilon^2}{8\lambda}
\end{align*}

==> primitive_exp.tex <==

\mypara{Exponential Mechanism}
The exponential mechanism (EM)~\cite{focs:mcsherry07} samples from the set of all possible answers according to an exponential distribution, with answers that are ``more accurate'' being sampled with higher probability.  
% \says{Ninghui}{Since a function can take one or more arguments, it really should be one function that assignes a quality score to each value.  Also, don't use the word index here, since it has not been defined.  It is specific to this problem, but here we are describing EM as a general mechanism.}
This approach requires the specification of a quality function $q$ that takes as input the data $V$, a possible output $o$, and outputs a real-numbered quality score. 
% \says{zhikun}{why there are a set of quality functions?}.
% $\mathcal{V} \rightarrow \mathbb{R}$.  
% This makes it consistent with NoisyMax and SVT (in fact, I believe they can be generalized) } 
% where the real valued score $q(V,r)$ indicates how accurate it is to return $r$ when the input is $V$.  Higher scores indicate more accurate outputs which should be returned with higher probabilities.  
% Given the quality function $q$, its global sensitivity $\mathsf{GS}_q$ is defined as:
% $$ \mathsf{GS}_q = \max_{r} \max_{(V,V'):d(V, V')=1} |q(V,r) - q(V',r)| $$
% The following method $\AA$ satisfies $\epsilon$-differential privacy:
% \begin{equation}
%  \Pr{\AA_q(V)=r} \propto \exp{\left(\frac{\epsilon }{2\,\mathsf{GS}_q}q(V,r)\right)} \label{eq:exp}
% \end{equation}
The global sensitivity of the quality functions $\mathsf{GS}_q$ is defined as:
\begin{align}
    \mathsf{GS}_q = \max_{o} \max_{V\simeq V'} |q(V,o) - q(V',o)|
    % \nonumber
    \label{eq:gs_exp}
\end{align} 
The following method $\AA$ satisfies $\epsilon$-differential privacy:
% \begin{align}
%  \Pr{\AA_q(V)=i} \propto \exp{\left(\frac{\epsilon }{2\,\mathsf{GS}_q}q_i(V)\right)} \label{eq:exp}
% \end{align}
\begin{align}
 \Pr{\AA_q(V)=o} =\frac{ \exp{\left(\frac{\epsilon }{2\,\mathsf{GS}_q}q(V,o)\right)}}{\sum_o' \exp{\left(\frac{\epsilon }{2\,\mathsf{GS}_q}q(V,o')\right)}} \label{eq:exp}
\end{align}

As shown in EM~\cite{focs:mcsherry07}, if the quality function satisfies the condition that when the input dataset is changed from $V$ to $V'$, the quality scores of all outcomes change in the same direction, i.e., for any neighboring $V$ and $V'$
\[
\left(\exists_o\, q(V,o) \!<\! q(V',o)\right) \!\implies\! \left(\forall_{o'}\,q(V,o') \!\leq \! q(V',o')\right)
\]

Then one can remove the factor of $1/2$ in the exponent of \autoref{eq:exp} and return $i$ with probability proportional to $\exp\!{\left(\frac{\epsilon }{\mathsf{GS}_q}q(V,o)\right)}$.  This improves the accuracy of the result.



Recently, McKenna and Sheldon~\cite{nips20:mckenna2020permute} improves EM by replacing the sampling method from \autoref{eq:exp} to a sequential flipping method.  We present the details of it in \autoref{app:dp_primitive}.
% \zzk{Shall we give it a name here such as PF if we want to use it later?}
% \tw{I give it a name later; here let's keep the reader's mental load low}




==> primitive_gau.tex <==
\mypara{Gaussian Mechanism}
\label{subsubsec:gauss}
There are several approaches for designing mechanisms that satisfy $(\epsilon, \delta)$-differential privacy.  In this paper we use the Gaussian mechanism.  The approach computes a function $f$ on the dataset $V$ in a differentially privately way, by adding to $f(V)$ a random noise.  The magnitude of the noise depends on $\mathsf{GS}_f$, the \emph{global sensitivity} or the $L_2$ sensitivity of $f$.  Such a mechanism $\AA$ is given below:
$$
\begin{array}{crl}
& \AA(V) & =f(V)+\calN\left(\frac{\sqrt{2\ln(1.25/\delta)}\cdot \mathsf{GS}_f }{\epsilon} \right)
  \\
\mbox{where} &  \mathsf{GS}_f & = \max\limits_{V \simeq V'} ||f(V) - f(V')||_2,
\\
\mbox{and}& \Pr{\calN\left(\sigma \right)=x} & = \frac{1}{\sqrt{2\pi\sigma}} \myexp{-x^2/2\sigma^2}
\end{array}
$$
In the above, $\calN (\sigma)$ denotes a random variable sampled from the normal distribution with mean $0$ and standard deviation $\sigma$.
As $\calN (\sigma)$ is zero-mean, $\AA(V)$ is a natural (unbiased) estimator of $f(V)$.

==> primitive_grr.tex <==

\mypara{Generalized Randomized Response}
\label{subsubsec:rr}
% The Gaussian Mechanism can also be applied to ensure LDP, by adding noise $\calN (0, \mathsf{GS}_f^2\cdot \sigma^2 )$ to each single result $f(D) = f(\{v\})$ (e.g., as in~\cite{zheng2017collect}). 
% But for the same (or even better, as Gaussian mechanism have $\delta>0$) privacy guarantee, there exist other mechanisms that gives better utility.  
The basic mechanism in LDP is called randomized response~\cite{jasa:Warner65}.  It was introduced for the binary case, but can be easily generalized to the categorical setting.  Here we describe the generalized version of random response (\grr for short).
%, which enables the estimation of the frequency of any given value $v\in \Domain$.

In \grr, each user with private value $v$ sends $\grr(v)$ to the server, where $\grr(v)$ outputs the true value $v$ with probability $p$, and a randomly chosen value $v'\ne v$ with probability $1-p$.  All values are in a pre-defined domain $\Domain$ of size $d=|\Domain|$.
The perturbation function is defined as
\begin{align}
\forall_{y \in \Domain}\;\Pr{\grr(v) = y}  = \left\{
\begin{array}{lr}
p=\frac{e^\epsilon}{e^\epsilon + d - 1}, & \mbox{if} \; y = v  \\
q= \frac{1}{e^\epsilon + d - 1}, & \mbox{if} \; y \neq v \\
\end{array}\label{eq:grr}
\right.
\end{align}
This satisfies $\epsilon$-LDP since $\frac{p}{q}=e^\epsilon$.  
% Unlike Gaussian mechanism, which adds unbiased noise, random response is asymmetric, and to estimate the frequency of $v\in \Domain$ (i.e., the ratio of the users who have $v$ as private value to the total number of users), one needs to count how many times $v$ is reported, denote by $C(v)$, and then computes
Different from the Laplace mechanism, the result of \grr needs to be calibrated.  That is, to estimate the frequency of $\tilde{f}_v$ for $v\in \Domain$, one counts how many times $v$ is reported, denoted by $\sum_{i\in[n]}\ind{y_i=v}$, and then computes
\begin{align}
\tilde{f}_v =  \frac{1}{n}\sum_{i\in[n]}\frac{\ind{y_i=v}-q}{p-q} \label{eq:grr_aggregate}
\end{align}
where $\ind{y_i=v}$ is the indicator function that the report of the $i$-th user $y_i$ equals $v$, and $n$ is the total number of users.

==> primitive_olh.tex <==

\mypara{Optimal Local Hashing}
When $d$ is large, the $p$ value in Equation~\eqref{eq:grr} becomes small, making the result inaccurate.  
% To overcome this issue, the local hashing idea~\cite{stoc:BassilyS15} let each user map $v$ to one bit, and then use \grr to perturb it.  More formally, each user reports $\tuple{H,\grr(H(v))}$ to the server, where $H$ is the mapping (hashing) function.
% In this protocol, both the hashing step and the randomization step result in information loss.  Later, Wang et al.~\cite{uss:WangBLJ17} realized $H$ does not necessarily hash $v$ to one bit.  In fact, the output domain size $d'$ of $H$ is a tradeoff.  The optimal $d'$ is $e^\epsilon+1$.  And the method is called Optimized Local Hash (\olh).
% This protocol deals with a large domain size $d=|\Domain|$ by first using a hash function to compress the input domain into a smaller domain of size $d' < d$, and then applying randomized response to the hashed value.  
To overcome this issue, the optimal local hashing (\olh) lets each user map $v$ to a smaller domain of size $d'=e^\epsilon+1$ and use \grr to perturb it.  More formally, each user reports $\tuple{H,\grr(H(v))}$ to the server, where $H$ is the mapping (hashing) function.
% In this protocol, both the hashing step and the randomization step result in information loss.  Later, Wang et al.~\cite{uss:WangBLJ17} realized $H$ does not necessarily hash $v$ to one bit.  In fact, the output domain size $d'$ of $H$ is a tradeoff.  The optimal $d'$ is $e^\epsilon+1$.  And the method is called Optimized Local Hash (\olh).
% loss of information during the hashing step and loss of information during the randomization step.  

% More formally, each user reports $\tuple{H,\grr(H(v))}$ where $H$ is randomly chosen from a family of hash functions that hash each value in $\Domain$ to $\{1\ldots d'\}$, and $\grr(\cdot)$ is the perturbation function for random response, while operating on the domain $\{1\ldots d'\}$ (thus $p = \frac{e^\epsilon}{e^\epsilon+d'-1}$ in Equation~\eqref{eq:grr}).
Similar to \grr, the result of \olh needs to be calibrated.  Let $\tuple{H_i,y_i}$ be the report from the $i$'th user.
For each value $v\in \Domain$, to compute its frequency, one first computes $|\{i\mid H_i(v) = y_i\}| = \sum_{i\in[n]}\ind{ H_i(v) = y_i}$, 
and then transforms it to its unbiased estimation
\begin{align}
\tilde{f}_v = \frac{1}{n}\sum_{i\in[n]}\frac{\ind{ H_i(v) = y_i} - 1/d'}{p - 1/d'}\label{eq:olh_aggregate}
\end{align}

% In~\cite{wang2017locally}, by minimizing the estimation variance, $d'$ is optimized as $e^\epsilon+1$.  The method is called Optimized Local Hashing (\olh).
%suggested that setting $d'$ to be the nearest integer of $e^\epsilon+1$ gives minimal variance~\cite{wang2017locally}.
% In~\cite{wang2017locally}, the estimation variances of \grr and \olh are analyzed and compared.  
% The variance of this estimation is
% \begin{align*}
% % \label{eq:var_olh}
% \mathrm{Var}[\tilde{x}_v]=\frac{4e^\epsilon}{(e^\epsilon-1)^2\cdot n}.
% \end{align*}
% Compared with \eqref{var_grr}, the factor $d-2+e^\epsilon$ is replaced by $4 e^\epsilon$.  This suggests 
% \says{tianhao}{todo}
% Unlike \grr, \olh has a variance that does not depend on $|\Domain|$.  As a result, 
It is shown in~\cite{uss:WangBLJ17} that for a smaller domain size ($|\Domain|-2<3e^\epsilon$), \grr is better; but for larger $|\Domain|$, \olh is preferable. 


% To handle high-dimensional cases, one can construct a domain that is the Cartesian product of the domains for each dimension.  We focus on one-dimensional data in this work; our analysis and evaluations can be easily generalized to multi-dimensional data.

% \cite{sigmod:WangDZHHLJ19} proposes an algorithm based on one-dimensional LDP mechanisms, called frequency oracles, to handle multi-dimensional range queries accurately. The accuracy of these algorithms fundamentally depends on the underlying LDP mechanisms, and, therefore, even though we focus on one-dimensional data in this work, our analysis and evaluations can be easily generalized to multi-dimensional data.

==> primitive_pf.tex <==

\mypara{Permute-and-flip Mechanism}
The permute-and-flip mechanism (PF)~\cite{:} samples from the set of all possible answers according to an exponential distribution, with answers that are ``more accurate'' being sampled with higher probability.  
This approach requires the specification of a quality functions $q$ that takes as input the data $V$, a possible output $o$, and outputs a real-numbered quality score. 
The global sensitivity of the quality functions $\mathsf{GS}_q$ is defined as:
\begin{align}
    \mathsf{GS}_q = \max_{o} \max_{V\simeq V'} |q(V,o) - q_i(V',o)|
    % \nonumber
    \label{eq:gs_exp}
\end{align} 
The following method $\AA$ satisfies $\epsilon$-differential privacy:
\begin{align}
 \Pr{\AA_q(V)=o} =\frac{ \exp{\left(\frac{\epsilon }{2\,\mathsf{GS}_q}q(V,o)\right)}}{\sum_o' \exp{\left(\frac{\epsilon }{2\,\mathsf{GS}_q}q(V,o')\right)}} \label{eq:exp}
\end{align}

As shown in~\cite{focs:mcsherry07}, if the quality function satisfies the condition that when the input dataset is changed from $V$ to $V'$, the quality scores of all outcomes change in the same direction, i.e., for any neighboring $V$ and $V'$
\[
\left(\exists_o\, q(V,o) \!<\! q(V',o)\right) \!\implies\! \left(\forall_{o'}\,q(V,o') \!\leq \! q(V',o')\right)
\]

Then one can remove the factor of $1/2$ in the exponent of Equation~(\ref{eq:exp}) and return $i$ with probability proportional to $\exp\!{\left(\frac{\epsilon }{\mathsf{GS}_q}q(V,o)\right)}$.  This improves the accuracy of the result.

==> primitive_zcdp.tex <==
\mypara{Advanced Composition}
\label{subsubsec:zcdp}
For a sequential of $k$ mechanisms $\AA_1, \ldots, \AA_k$ satisfying $(\epsilon_i, \delta_i)$-DP for $i=1,\ldots, k$ respectively, the basic composition result~\cite{dpbook} shows that the privacy composes linearly, i.e., the sequential composition satisfies $(\sum_i^k\epsilon_i, \sum_i^k\delta_i)$-DP. When $\epsilon_i=\epsilon$ and $\delta_i=\delta$, the advanced composition bound provided by Dwork et al.~\cite{focs:dwork2010boosting} states that the composition satisfies ($\epsilon \sqrt{2k\log(1/\delta')}+k\epsilon(e^\epsilon-1)$, $k\delta+\delta'$)-DP. 

\mypara{Composition via Zero-Concentrated DP}
To enable more complex algorithms and data analysis task via the composition of multiple differentially private building blocks, zero Concentrated Differential Privacy (\zcdp for short) offers an elegant composition property that is even stronger than advanced composition. 
In particular, \zcdp is defined with R\'enyi divergence:
\begin{definition}[Zero-Concentrated Differential Privacy (\zcdp)~\cite{tcc:bun2016concentrated}]
A randomized mechanism $\AA$ is $\rho$-zero concentrated differentially private (i.e., $\rho$-\zcdp) if for any two neighboring databases $V$ and $V'$ and all $\alpha \in (1, \infty)$,
\begin{align*}
\mathcal{D}_\alpha (\AA(V)||\AA(V')) \overset{\Delta}{=} \frac{1}{\alpha -1} \log \big(\mathbb{E}\left[ e^{(\alpha-1)L^{(o)}} \right] \big) \le \rho \alpha 
\end{align*}
Where $\mathcal{D}_\alpha (\AA(V)||\AA(V'))$ is called $\alpha$-R\'enyi divergence between the distributions of $\AA(V)$ and $\AA(V')$.
\end{definition}


\zcdp has a simple linear composition property~\cite{tcc:bun2016concentrated}:
\begin{prop}
\label{prop:zcdp-compose}
Two randomized mechanisms $\AA_1$ and $\AA_2$ satisfy $\rho_1$-\zcdp and $\rho_2$-\zcdp respectively, their sequential composition  $\AA = (\AA_1,\AA_2)$ satisfies ($\rho_1+\rho_2$)-\zcdp.
\end{prop}

The following two propositions restate the results given by Bun and Steinke~\cite{tcc:bun2016concentrated}, which are useful for composing Gaussian mechanisms in differential privacy.

\begin{prop} \label{prop:CDPtoDP}
If $\AA$ provides $\rho$-\zcdp, then $\AA$ is $(\rho+2\sqrt{\rho\log(1/\delta)},\delta)$-differentially private for any $\delta>0$.
\end{prop}

\begin{prop}
\label{prop:Gaussian-zcdp}
The Gaussian mechanism which answers $f(V)$ with noise $\calN(0, \mathsf{GS}_f^2 \sigma^2 \mathbf{I})$ satisfies ($\frac{1 }{2\sigma^2}$)-\zcdp.
\end{prop}


Given the privacy constraint $\epsilon$ and $\delta$, we can calculate the amount of noise for each task using \autoref{prop:zcdp-compose} to~\autoref{prop:Gaussian-zcdp}.  
In particular, we first use \autoref{prop:CDPtoDP} to compute the total $\rho$ allowed.  Then we use \autoref{prop:zcdp-compose} to allocate $\rho_i$ for each task $i$. Finally, we use \autoref{prop:Gaussian-zcdp} to calculate $\sigma$ for each task. Note that there are other techniques that gives the same composition results~\cite{csf:mironov2017renyi,arXiv:dwork2016concentrated}; we use \zcdp because it is the most convenient one.
% \says{jc}{not correctly displayed}\tw{what is not correctly displayed?}
% Compared with $(\epsilon, \delta)$-DP, \zcdp provides a tighter bound on the cumulative privacy loss under composition, making it more suitable for algorithms consist of a large number of tasks. 


